Unlocking Temporal Question Answering for Large Language Models with Tailor-Made Reasoning Logic

The temporal aspect is a significant dimension of our reality. We notice the challenge that large language models (LLMs) face when engaging in temporal reasoning. Our preliminary experiments show that methods involving the generation of intermediate reasoning steps, such as chain-of-thought and program-aided language models, do not consistently boost the performance of complex temporal question-answering tasks. This limitation can be attributed to the LLMs' inadequate understanding of temporal information. To address this problem, we propose TempLogic, a novel framework designed specifically for temporal question-answering tasks across three levels of reasoning. TempLogic incorporates retrieval-guided context distillation, temporal data extraction, and tailor-made logic reasoning. Extensive experiments and analysis demonstrate the effectiveness of our framework in solving intricate time-bound reasoning tasks.

==> sections/7_limitations.tex <==
\section*{Limitations}
TempLogic leverages the capabilities of both large language models (LLMs) and a Python solver while employing retrieval-guided context distillation. The framework allows for the use of different coding languages during the script execution phase, a topic that will be thoroughly investigated in future research to provide a more comprehensive evaluation. Additionally, to ensure precise execution, predefined scripts are employed for each dataset. Going forward, alternative approaches will be explored to automatically generate scripts, expanding the flexibility and adaptability of the framework. Moreover, the scope of exploration will extend beyond temporal reasoning question-answering, encompassing other symbolic tasks.


==> sections/8_ethical_impact.tex <==
\section*{Ethical Impact}

==> tbls/algo.tex <==
\begin{algorithm*}
    \caption{TempoRexx}
    \label{alg:ve}
    \begin{algorithmic}
        \Require $\textrm{Question } q$, $\textrm{context } c$, $\textrm{instruction prompt for information extraction } p_{extract}$;
        \Require $\textrm{Retrieval system } R(\cdot)$; $\textrm{Sentence embedding model } e(\cdot)$;
        \Require $\textrm{LLM } f(\cdot)$; $\textrm{LM decoding temperature } \tau$, $\textrm{Python solver } h(\cdot)$

        \State $D \gets R(q_i)$ \Comment{Retrieved information}
        \For{$d_i$ in $D$} \Comment{Top three similar sentences in context for each retrieved sentence}
            \State $T_i \gets \{c_1, c_2, c_3\}, \cos(e(d_i),e(c_1))>\cos(e(d_i),e(c_2))>\cos(e(d_i),e(c_3))>\dots$ 
        \EndFor
        \State $s \gets T_1 \cup T_2\dots\cup T_n$ \Comment{Combine unique distilled sentences as distilled context}

        \State $R, I \gets f(q, s, p_{extract}, \tau)$ \Comment{Extracted reference object (R) and structural information (I).}
        \State $A \gets h(R, I)$ \Comment{Execute code to get final answer (A).}
        \\ \Return{A}


    \end{algorithmic}
\end{algorithm*}

==> tbls/step2_code.tex <==
% \begin{lstlisting}[language=Python]
% import numpy as np
    
% def incmatrix(genl1,genl2):
%     m = len(genl1)
%     n = len(genl2)
%     M = None #to become the incidence matrix
%     VT = np.zeros((n*m,1), int)  #dummy variable
    
%     #compute the bitwise xor matrix
%     M1 = bitxormatrix(genl1)
%     M2 = np.triu(bitxormatrix(genl2),1) 

%     for i in range(m-1):
%         for j in range(i+1, m):
%             [r,c] = np.where(M2 == M1[i,j])
%             for k in range(len(r)):
%                 VT[(i)*n + r[k]] = 1;
%                 VT[(i)*n + c[k]] = 1;
%                 VT[(j)*n + r[k]] = 1;
%                 VT[(j)*n + c[k]] = 1;
                
%                 if M is None:
%                     M = np.copy(VT)
%                 else:
%                     M = np.concatenate((M, VT), 1)
                
%                 VT = np.zeros((n*m,1), int)
    
%     return M
% \end{lstlisting}


\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{0mm}{
            \begin{tabular}{p{8cm}}
            \toprule
                \texttt{\textbf{from} datetime \textbf{import} datetime}\\
                \texttt{extracted\textunderscore info = \textcolor{myred}{$ri_i$}}\\
                \texttt{ref\textunderscore obj = \textcolor{myred}{$ro_i$}}\\\\

                \texttt{\textbf{def} solution():}\\
                \texttt{\hspace{0.5cm} \textcolor{myred}{\#Code implementation...}}\\
                \texttt{\textbf{return} answer}\\
                \texttt{\textbf{print(solution())}} \\
            \bottomrule
            \end{tabular}
        }}
    \caption{
        Prompt for the second step in our framework: code execution. 
        Text in \textcolor{myred}{red}: the extracted\textunderscore info and ref\textunderscore obj, and code implementation of the corresponding temporal question-answering task. 
    }
    \label{tab:step2_code}
\end{table}

